UVLLM: An Automated Universal RTL Verification Framework using LLMs

Verifying hardware designs in embedded systems is crucial but often labor-intensive and time-consuming. While existing solutions have improved automation, they frequently rely on unrealistic assumptions. To address these challenges, we introduce a novel framework, UVLLM, which combines Large Language Models (LLMs) with the Universal Verification Methodology (UVM) to relax these assumptions. UVLLM significantly enhances the automation of testing and repairing error-prone Register Transfer Level (RTL) codes, a critical aspect of verification development. Unlike existing methods, UVLLM ensures that all errors are triggered during verification, achieving a syntax error fix rate of 86.99% and a functional error fix rate of 71.92% on our proposed benchmark. These results demonstrate a substantial improvement in verification efficiency. Additionally, our study highlights the current limitations of LLM applications, particularly their reliance on extensive training data. We emphasize the transformative potential of LLMs in hardware design verification and suggest promising directions for future research in AI-driven hardware design methodologies. The Repo. of dataset and code: https://anonymous.4open.science/r/UVLLM/.

==> RelatedWork.tex <==
\vspace{-2.5pt}
\section{Related Work}
\label{sc:RelatedWork}
\vspace{-2.5pt}

Recent advances in LLMs have significantly transformed hardware design, primarily through enhanced efficiency and automation~\cite{liu2023verilogeval,thakur2023verigen,blocklove2023chip, delorenzo2024make}. A key application of these models is in RTL debugging, which represents a substantial portion of total design costs. In response, various approaches, such as RTLFixer~\cite{tsai2023rtlfixer}, SBF~\cite{ahmad2023fixing}, LLM4SecHW~\cite{fu2023llm4sechw}, HDLdebugger~\cite{yao2024hdldebugger}, and AssertLLM~\cite{fang2024assertllm}, have been developed to reduce costs and increase efficiency in this area. 

These existing approaches have focused mainly on refining LLM models' performance by employing techniques like prompt engineering~\cite{white2023prompt,sahoo2024systematic}, model tuning~\cite{liu2023verilogeval,chang2023chipgpt}, and model training~\cite{liu2023chipnemo,goh2024english}. Although these efforts have led to some improvements, they have not yet successfully addressed applications to correcting function errors~\cite{ tian2024debugbench} nor achieved sufficient performance as measured by the \emph{pass@k} rates~\cite{ tsai2023rtlfixer}. In contrast, our approach adopts a collaborative process, by utilising two LLM models iteratively, to enhance debugging effectiveness for syntax and function errors.  


% The recent advancements in Large Language Models (LLMs) have demonstrated considerable potential in code generation as well as in automated debugging tasks, which have recently garnered considerable interest from researchers.

% One noteworthy development is the RTLFixer framework\cite{tsai2023rtlfixer} presented by YunDa et al. (2023). This framework employs LLMs to automatically correct syntax errors in Verilog code. By employing a combination of RAG and ReAct prompting mechanisms, RTLFixer enables the LLMs to operate as autonomous debugging agents, resulting in significant efficiency improvements. The framework demonstrated its effectiveness by achieving a 98.5\% success rate in correcting compilation errors, substantially enhancing the pass@k in benchmark datasets. This approach exemplifies the integration of human expertise with autonomous machine learning models to refine debugging processes in hardware design. 

% Building on this syntax-focused approach, the LLM4SecHW framework\cite{fu2023llm4sechw} leverages domain-specific LLMs to detect and rectify security vulnerabilities within hardware designs, showcasing the potential of fine-tuned LLMs in specialized fields beyond general syntax errors. 

% Similarly, the HDLdebugger project\cite{yao2024hdldebugger} extends the application of LLMs to streamline the debugging of hardware description languages, contributing to the reduction of manual debugging efforts and enhancing the development workflow. 

% Meanwhile, the study on hardware security bugs fixing with LLMs\cite{ahmad2023fixing} underscores the possible role of LLMs in preemptively identifying and patching security flaws in hardware, enhancing the overall reliability and security of hardware systems. 

% Collectively, these developments illustrate a growing trend towards the integration of LLM capabilities in both the identification and correction of a broad range of hardware-related errors. Although LLM has the potential to be an effective tool for error handling, there are still limitations in its ability to address functional errors and achieve high-quality code. Take RTLfixer as an instance, for the pass@k metric, only a 16\% correction was achieved on the RTLLM dataset.

% Complementing previous focus on syntax errors only, the DebugBench benchmark\cite{tian2024debugbench} introduced by Runchu et al. (2024) evaluates the LLMs' capabilities to debug both syntax and function errors across multiple programming languages, including C++, Java, and Python. DebugBench is meticulously constructed with over 4,000 instances encompassing a wide range of bug types, providing a comprehensive testing ground for assessing the effectiveness of the LLMs in identifying and correcting complex and diverse programming errors. This benchmark measures the performance of both commercial and open-source LLMs, revealing insights into their ability to handle the multifaceted challenges presented by both syntax discrepancies and function inaccuracies. It has been demonstrated that the LLMs are capable of achieving higher function error correction rates through iteration.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%One noteworthy development is the RTLFixer framework\cite{tsai2023rtlfixer} presented by YunDa et al. (2023). This framework employs LLMs to automatically correct syntax errors in Verilog code. By employing a combination of Retrieval-Augmented Generation (RAG) and ReAct prompting mechanisms, RTLFixer enables the LLMs to operate as autonomous debugging agents, resulting in significant efficiency improvements. The framework demonstrated its effectiveness by achieving a 98.5\% success rate in correcting compilation errors, substantially enhancing the first-pass success rates in benchmark datasets. This approach exemplifies the integration of human expertise with autonomous machine learning models to refine debugging processes in hardware design. However, the work focuses only on debugging of syntax error, and for the pass@k metric, only a 16\% correction was achieved on the RTLLM dataset.

==> ToDoList.tex <==
To do list:

1) Extensions: snippets of code(also logs)

2) Extensions: bug location

3) Extensions: UVM framework inspired

4) Extensions: testbench with SystemC (future work if not in time)

5) Extensions: datasets (junhao)
%2) Fix rate: 93\% Syntax, Functional 78\%, pass@1 (Delete); Speedup 6/7x -- Jialin
%3) Size of Table 5: i) change the absolute numbers to percentage; 2) change 1, 2, to S and F -- Zhe Jiang (Table size); Jialin (Contents)
%4) Syntax error v.s. function error - Zhe Jiang
%5) Table 1, examples of correct and errors --- Yuchen



%British English -- Zhe Jiang done

%Tense -- Zhe Jiang  

%log v.s. logs -- Zhe Jiang 


%function v.s. functional -- Xuke 
%syntax v.s. syntatic -- Xuke

